Instructive Decoding: Instruction-Tuned Large Language Models are Self-Refiner from Noisy Instructions

While instruction-tuned language models have demonstrated impressive zero-shot generalization, these models often struggle to generate accurate responses when faced with instructions that fall outside their training set. This paper presents Instructive Decoding (ID), a simple yet effective approach that augments the efficacy of instruction-tuned models. Specifically, ID adjusts the logits for next-token prediction in a contrastive manner, utilizing predictions generated from a manipulated version of the original instruction, referred to as a noisy instruction. This noisy instruction aims to elicit responses that could diverge from the intended instruction yet remain plausible. We conduct experiments across a spectrum of such noisy instructions, ranging from those that insert semantic noise via random words to others like 'opposite' that elicit the deviated responses. Our approach achieves considerable performance gains across various instruction-tuned models and tasks without necessitating any additional parameter updates. Notably, utilizing 'opposite' as the noisy instruction in ID, which exhibits the maximum divergence from the original instruction, consistently produces the most significant performance gains across multiple models and tasks.

==> materials/tables/table_few_shot.tex <==
\begin{wraptable}{r}{0.4\textwidth}
\centering
\vspace{-10pt}
\caption{Rouge-L scores under a few-shot scenario across different models. We set $\epsilon$ to 0.2.}
\label{tab:few-shot}
\vspace{-5pt}
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{cccc}
\toprule
Method & Tk-Large & Tk-XL & Alpaca-7b \\
\midrule
baseline & 47.63&	54.34&	37.06\\
null & 47.94&	54.78&	38.75\\
null$^*$ &46.95&	54.41&	38.07\\
opposite & 48.08&	54.80&	37.79\\
opposite$^*$ & 47.01&	54.51&	 37.55\\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{wraptable}


==> materials/tables/table_noisy_examples.tex <==
\begingroup
\setlength{\tabcolsep}{3.5pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.06}
\begin{table}[ht!]
\centering
\caption{Examples of misleading instances included in the \textsc{SupNatInst} dataset. The misleading part is highlighted in \textcolor{red}{red}, along with explanations for why it is misleading.}
\begin{tabular}{@{}ll}
\toprule
\textbf{Task ID}
& task199\_mnli\_classification
\\
\hline
\textbf{Instance ID} 
& task199-9f3e5f6241ce41c7ba83bf9a2b6be11d
\\ 
\midrule
\textbf{Definition} 
& 
\begin{tabular}[c]{@{}l@{}}
In this task, you're given a pair of sentences, sentence 1 and sentence 2. Your \\job is to determine if the two sentences clearly agree/disagree with each other, \\or if this can't be determined. Indicate your answer as yes or no respectively.
\end{tabular}
\\ 
\midrule
\textbf{Instance}
&
\begin{tabular}[c]{@{}l@{}}
Sentence 1: Ninety-five percent of the total amount of sulfur dioxide \\allowances allocated each year under Section 423 will be allocated based on \\the amount of sulfur dioxide allowances allocated under the Acid Rain Program \\for 2010 and thereafter and that are held in allowance accounts in the Allowance \\Tracking System on the date 180 days after enactment. Sentence 2: Most of the \\sulfur dioxide that is allowed are controlled by the Acid Rain Program.
\end{tabular} 
\\
\midrule
\textbf{Golden Labels}
&
\begin{tabular}[c]{@{}l@{}}
[\textcolor{red}{"no"}, "yes"] \textcolor{red}{\qquad\# An additional incorrect label is included.}
\end{tabular}
\\
\hline\hline
\textbf{Task ID}
& task020\_mctaco\_span\_based\_question
\\
\midrule
\textbf{Instance ID} 
& task020-3b643de54d474381854c2499cd185a74
\\ 
\midrule
\textbf{Definition} 
& 
\begin{tabular}[c]{@{}l@{}}
The answer will be 'yes' if the provided sentence contains an explicit mention \\that answers the given question. Otherwise, the answer should be 'no'. Instances \\ where the answer is implied from the sentence using "instinct" or "common \\sense" (as opposed to being written explicitly in the sentence) should be labeled \\as 'no'.
\end{tabular}
\\ 
\midrule
\textbf{Instance}
&
\begin{tabular}[c]{@{}l@{}}
Sentence: Jerry goes out to the pier and casts his favorite bait : cheese .  
\\
Question: How much time did Jerry spend at the pier?
\end{tabular} 
\\
\midrule
\textbf{Golden Labels}
&
\begin{tabular}[c]{@{}l@{}}
[\textcolor{red}{"No."}] \textcolor{red}{\qquad\# Unexpected capital letter and period are included.}
\end{tabular} 
\\
\hline\hline
\textbf{Task ID}
& task738\_perspectrum\_classification
\\
\midrule
\textbf{Instance ID} 
& task738-7bde66d008f6449f90b430dac8a78257
\\ 
\midrule
\textbf{Definition} 
& 
\begin{tabular}[c]{@{}l@{}}
In this task you will be given a claim and a perspective. You should determine \\whether that perspective \textcolor{red}{supports} or \textcolor{red}{undermines} the claim. If the perspective \\could possibly convince someone with different view, it is \textcolor{red}{supporting}, otherwise \\it is \textcolor{red}{undermining}.
\end{tabular}
\\ 
\midrule
\textbf{Instance}
&
\begin{tabular}[c]{@{}l@{}}
claim: Domestic intelligence agencies have a legitimate role to play in democracy.
\\
perspective: The government does not have the right to spy on its citizens
\end{tabular} 
\\
\midrule
\textbf{Golden Labels}
&
\begin{tabular}[c]{@{}l@{}}
[\textcolor{red}{"undermine"}] \textcolor{red}{\qquad\# The label space is ambiguously defined.}
\end{tabular} 
\\
\hline\hline
\textbf{Task ID}
& task1624\_disfl\_qa\_question\_yesno\_classification
\\
\midrule
\textbf{Instance ID} 
& task1624-ef6dff90c9ae4c5fb513d3e0c4f16f19
\\ 
\midrule
\textbf{Definition} 
& 
\begin{tabular}[c]{@{}l@{}}
In this task you are given a disfluent question, a proper question and a context. \\ A disfluent question is a question that has some interruptions in it while framing \\and a proper question is the correct form of the question without any disfluency. \\\textcolor{red}{Classify whether the question is answerable or not} based on the given context.
\end{tabular}
\\ 
\midrule
\textbf{Instance}
&
\begin{tabular}[c]{@{}l@{}}
proper question: Who was the last known European to visit China and return? 
\\disfluent question: What did Polo, no I'm sorry, who was the last known European to 
\\ visit China and return? 
\\context: The first recorded travels by Europeans to China and back date from this time. \\The most famous traveler of the period was the Venetian Marco Polo, \textit{\textcolor{gray}{... \{Skip\}...}}\\Some suggest that Marco Polo acquired much of his knowledge through contact with \\Persian traders since many of the places he named were in Persian.
\end{tabular} 
\\
\midrule
\textbf{Golden Labels}
&
\begin{tabular}[c]{@{}l@{}}
[\textcolor{red}{"No"}] \textcolor{red}{\qquad\# The explicit label space is not defined.}
\end{tabular}
\\
\bottomrule
\end{tabular}
\\
\end{table}
\endgroup


==> materials/tables/table_sni_balanced_classification.tex <==
\begin{table}[t]
\centering
\caption{Evaluation (mean \(\pm\) variance) on 58 classification tasks from the held-out dataset of \textsc{SupNatInst}.}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}c|ccc|ccc|ccc@{}}
\toprule
Model Size        & \multicolumn{3}{c}{770M} & \multicolumn{3}{c}{3B} & \multicolumn{3}{c}{11B} \\ \midrule
Evaluation Metric & EM                         & bACC                    & F1                     & EM                        & bACC                       & F1                       & EM                        & bACC                       & F1                       \\ \midrule
Standard          & 38.69 \(\pm\) 22.75        & 38.34 \(\pm\) 22.90      & 39.53 \(\pm\) 22.51     & 44.09 \(\pm\) 25.86       & 43.95 \(\pm\) 25.80         & 45.31 \(\pm\) 25.13      & 46.24 \(\pm\) 23.38       & 46.34 \(\pm\) 23.50         & 48.40 \(\pm\) 23.05       \\
Null              & 40.71 \(\pm\) 19.50         & 40.51 \(\pm\) 19.49     & 41.78 \(\pm\) 18.93     & 47.62 \(\pm\) 26.39       & 47.72 \(\pm\) 26.27        & 48.40 \(\pm\) 25.98       & 49.83 \(\pm\) 22.85       & 49.78 \(\pm\) 23.01        & 51.47 \(\pm\) 22.62      \\
Random Words      & 40.57 \(\pm\) 19.78        & 40.35 \(\pm\) 19.80      & 41.64 \(\pm\) 19.13     & 47.76 \(\pm\) 26.46       & 47.86 \(\pm\) 26.34        & 48.57 \(\pm\) 26.01      & 49.67 \(\pm\) 22.89       & 49.64 \(\pm\) 23.05        & 51.27 \(\pm\) 22.65      \\
Random Truncate   & 40.50 \(\pm\) 19.52         & 40.29 \(\pm\) 19.51     & 41.58 \(\pm\) 18.90      & 47.29 \(\pm\) 26.16       & 47.39 \(\pm\) 26.04        & 48.12 \(\pm\) 25.68      & 50.02 \(\pm\) 22.41       & 49.96 \(\pm\) 22.57        & 51.40 \(\pm\) 22.29       \\
Opposite          & 39.97 \(\pm\) 19.97        & 39.68 \(\pm\) 20.09     & 41.13 \(\pm\) 19.20      & 47.59 \(\pm\) 25.59       & 47.70 \(\pm\) 25.48         & 48.50 \(\pm\) 25.13       & 50.47 \(\pm\) 22.93       & 50.48 \(\pm\) 23.08        & 51.96 \(\pm\) 22.77      \\ \bottomrule
\end{tabular}%
}
\end{table}

==> materials/tables/table_sni_noisy_benchmark.tex <==
\begin{table}[h!]
    \centering
    \caption{The zero-shot performance of noisy instructions on unseen tasks in the test set of \textsc{SupNatInst} \citep{sni_dataset} is evaluated using Tk-instruct 3b. We report Rouge-L as our aggregated metric.}
    \label{tab:sni_noisy_benchmark}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{@{}cccccccccccccc@{}}
        \toprule
        Method & Overall & AC & CE & CR & DT & DAR & GEC & KT & OE & QR & TE & TG & WA \\
        \midrule
        baseline & 41.10&	55.95&	54.33&	38.32&	30.53&	40.72&	86.06&	51.16&	27.30&	55.19&	42.18&	31.31&	12.21 \\
        \midrule
        shuffle & 30.89&	40.76&	45.67&	31.07&	26.47&	29.97&	77.88&	34.34&	14.33&	28.13&	33.18&	23.71&	16.02\\
        trunc-0.6 & 28.57&	29.62&	38.55&	31.73&	28.07&	25.25&	78.01&	41.14&	12.90&	30.25&	26.87&	26.24&	13.83\\
        trunc-0.8 & 19.68&	16.54&	22.62&	24.13&	24.52&	14.85&	54.80&	29.21&	16.39&	21.49&	14.99&	21.28&	12.13\\
        null & 13.37&	2.07&	12.81&	22.11&	26.18&	3.24&	69.17&	25.40&	24.64&	9.50&	3.01&	22.31&	11.71\\
        rand words & 12.84&	2.17&	11.91&	21.52&	24.44&	3.07&	68.44&	24.49&	24.59&	9.87&	2.75&	21.48&	10.25\\
        opposite & 11.16&	3.19&	10.75&	18.58&	24.66&	1.55&	55.92&	18.43&	20.55&	16.11&	0.51&	16.04&	7.73\\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> materials/tables/table_unni_t0.tex <==
\begin{wraptable}{r}{0.38\textwidth}\small
\centering
\vspace{-10pt}
\caption{Overall Rouge-L scores across different models and datasets.}
\vspace{-5pt}
\label{tab:unni_t0}
\resizebox{0.38\textwidth}{!}{%
\begin{tabular}{cccc}
\toprule
\textbf{Dataset} & \textbf{\textsc{UnNatInst}} & \multicolumn{2}{c}{\textbf{\textsc{SupNatInst}}} \\
\midrule
\textbf{Model} & \textbf{Tk-Large} & \textbf{T0-3b} & \textbf{Alpaca-7b}\\
\midrule\midrule
baseline & 43.25 & 26.58 & 23.61\\
null & \textbf{44.57} & 29.33 & 31.21\\
random & 44.44 & \textbf{29.49} & 30.93\\
opposite & 43.42 & 29.46 & \textbf{31.38}\\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{wraptable}

==> materials/tables/table_usecases.tex <==
\begin{table}[]
\centering
\caption{An example task in the category AC and category WA of \textsc{Sup-NatInst}\,\citep{sni_dataset}.}
\label{tab:usecase}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lll@{}}
\toprule
Task Type                                                & Answerability Classification                             & Word Analogy                  \\ \midrule
Task ID                                                  & task1640\_adverserial\_qa\_answerability\_classification & task1156\_bard\_word\_analogy \\ \midrule
Instruction & 
  \begin{tabular}[c]{@{}l@{}}Given a paragraph from a wikipedia article about some topic, and a question related \\to the topic, determine whether the question is answerable from the paragraph. If \\the question is answerable,  answer ``True'', otherwise, answer ``False''.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Two analogies that relate actions to the tools \\used to perform the action is given in the form\\ “A : B. C : ?”. “A : B” relates action A to tool B. \\ Your task is to replace the question mark (?) with \\ the appropriate tool for the given action C,\\ following the “A : B” relation.\end{tabular} \\ \midrule
Instance &
  \begin{tabular}[c]{@{}l@{}}Input: In March 1971, the residential office of an FBI agent in Media, Pennsylvania \\was burglarized by a group calling itself the Citizens' Commission to Investigate \\the FBI. Numerous files were taken and distributed to a range of newspapers, including \\The Harvard Crimson. The files detailed the FBI's extensive COINTELPRO program, \\which included investigations into lives of ordinary citizens\u2014including a black \\student group at a Pennsylvania military college and the daughter of Congressman \\ Henry Reuss of Wisconsin. The country was \"jolted\" by the revelations, which included \\assassinations of political activists, and the actions were denounced by members of \\Congress, including House Majority Leader Hale Boggs. The phones of some members \\ of Congress, including Boggs, had allegedly been tapped. Question: Who was listening \\ to phone calls clandestinely?\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Input: stir : spoon. cut : ?\end{tabular} \\ \midrule
  \begin{tabular}[c]{@{}l@{}}Golden\\ Label\end{tabular} & True                                                          & {[}“scissors”, “sword”, “glass”, “knife”{]}\\ \midrule
\begin{tabular}[c]{@{}l@{}}$p(y|x)$ \\ (without Instruction)\end{tabular} & FBI                                                          & knife\\ \bottomrule          
\end{tabular} 
}
\end{table}

==> materials/tables_deprecated/table_decoding.tex <==
\begingroup
\setlength{\tabcolsep}{2.0pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.16}
\begin{table}[ht!]
\caption{Maybe we should evaluate across Model\&Scales rather than datasets?}
\centering
\begin{tabular}{lcccc} 
\toprule
\textbf{Methods}     & \multicolumn{1}{l}{\textbf{Nat. Inst}} & \multicolumn{1}{l}{\textbf{SupNat. Inst}} & \multicolumn{1}{l}{\textbf{Unnat. Inst}} & \multicolumn{1}{l}{\textbf{FLAN Collection}}  \\ 
\hline\hline
Baseline (Top-k, $tau$=1.0)     & 00.0                                   & 00.0                                      & 00.0                                     & 00.0                                          \\
\hline
Coherence Boosting   & 00.0                                   & 00.0                                      & 00.0                                     & 00.0                                          \\
NeuroLogic-a*        & 00.0                                   & 00.0                                      & 00.0                                     & 00.0                                          \\
Contrastive Decoding & 00.0                                   & 00.0                                      & 00.0                                     & 00.0                                          \\
SimCTG            & 00.0                                   & 00.0                                      & 00.0                                     & 00.0                                          \\
CAD                  & 00.0                                   & 00.0                                      & 00.0                                     & 00.0                                          \\ 
\hline
\textbf{MZ Decoding (Ours)}   & 00.0                                   & 00.0                                      & 00.0                                     & 00.0                                          \\
\bottomrule
\end{tabular}
\end{table}
\endgroup

\begingroup
\setlength{\tabcolsep}{6.0pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.1}
\begin{table}[ht!]
\caption{Maybe we should evaluate across Model\&Scales rather than datasets?}
\centering
\begin{tabular}{ccccc}
\toprule
\textbf{Methods}         & \textbf{Nat. Inst} & \textbf{SupNat. Inst} & \textbf{Unnat.Inst} & \textbf{FLAN Collection}  \\
\hline\hline
\textbf{Greedy}          & 00.0               & 00.0                  & 00.0                & 00.0                      \\
\multicolumn{1}{r}{+MZ}  & 00.0               & 00.0                  & 00.0                & 00.0                      \\
\textbf{Beam Search}          & 00.0               & 00.0                  & 00.0                & 00.0                      \\
\multicolumn{1}{r}{+MZ}  & 00.0               & 00.0                  & 00.0                & 00.0                      \\
\textbf{Top-k ($\tau$=1.0)}           & 00.0               & 00.0                  & 00.0                & 00.0                      \\
\multicolumn{1}{r}{+ MZ} & 00.0               & 00.0                  & 00.0                & 00.0                      \\
\textbf{Top-k ($\tau$=0.7)}           & 00.0               & 00.0                  & 00.0                & 00.0                      \\
\multicolumn{1}{r}{+ MZ} & 00.0               & 00.0                  & 00.0                & 00.0                      \\
\textbf{Nucleus}         & 00.0               & 00.0                  & 00.0                & 00.0                      \\
\multicolumn{1}{r}{+MZ}  & 00.0               & 00.0                  & 00.0                & 00.0                      \\
\bottomrule
\end{tabular}
\end{table}
\endgroup

==> materials/tables_deprecated/table_main.tex <==
\begingroup
\setlength{\tabcolsep}{2.0pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.16}
\begin{table}[ht!]
\caption{Zero-shot average ROUGE-L score across tasks.}
\centering
\begin{tabular}{ccclclclcl} 
\toprule
\multicolumn{2}{c}{\multirow{3}{*}{\textbf{Model }}} & \multicolumn{8}{c}{\textbf{Datasets}}                                                                                                               \\
\multicolumn{2}{c}{}                                 & \multicolumn{2}{c}{Nat. Inst}      & \multicolumn{2}{c}{SuperNat. Inst} & \multicolumn{2}{c}{Unnat. Inst}    & \multicolumn{2}{c}{FLAN Collection}  \\
\multicolumn{2}{c}{}                                 & w/o MZ & \multicolumn{1}{c}{w/ MZ} & w/o MZ & \multicolumn{1}{c}{w/ MZ} & w/o MZ & \multicolumn{1}{c}{w/ MZ} & w/o MZ & \multicolumn{1}{c}{w/ MZ}   \\ 
\hline\hline
\multirow{2}{*}{\textbf{T0 }}         & 3B           & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}                 \\
                                      & 11B          & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}                 \\
\multirow{2}{*}{\textbf{FLAN-T5 }}    & 3B           & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}                 \\
                                      & 11B          & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}                 \\
\multirow{2}{*}{\textbf{OPT-IML}}     & 1.3B         & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}                 \\
                                      & 30B          & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}                 \\
\multirow{2}{*}{\textbf{Tk-Instruct}} & 3B           & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}                 \\
                                      & 11B          & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}                 \\
\multirow{2}{*}{\textbf{Alpaca }}     & 7B           & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}                 \\
                                      & 13B          & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}                 \\
\multirow{2}{*}{\textbf{Vicuna}}      & 7B           & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}                 \\
                                      & 13B          & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}               & 00.0   & \textbf{00.0} \scriptsize{\textcolor{green!50!black}{(+ 0.0)}}                 \\
\bottomrule
\end{tabular}
\end{table}
\endgroup

==> materials/tables_deprecated/table_prompt_format.tex <==
\begin{table}[t]
\centering
\caption{Prompts for generating universality-enhanced instruction and conformity-enhanced instruction.}
\begin{tabular}{|p{13cm}|}\small
Your task is to separate the given original task instruction into two distinct instructions, Universiality Instruction and Conformity Instruction. You must follow the specified principles when splitting the original instructions into Universiality Instruction and Conformity Instruction.

Universality Principles:$\setminus$n
1. Core Objective Focus: Emphasize the primary goal or the essence of the task, deliberately avoiding specific procedures or answer formats. $\setminus$n
2. Broad Applicability: Frame the instruction in a manner that is universally understandable and can be applied across various scenarios.$\setminus$n
3. Holistic Contextualization: Use terms that encourage a broader, overall understanding of the task. Phrases like "in general" or "overall" may be helpful here.$\setminus$n
4. Open-Endedness: Allow for a range of possible solutions or methods to fulfill the task, avoiding limitations on specific answers.$\setminus$n$\setminus$n

Conformity Principles:$\setminus$n
1. Focused Directives: Lay out the exact steps or methods that need to be followed, providing a clear and singular pathway for execution.$\setminus$n
2. Format Specificity: Clearly articulate how the answer should be presented or formatted, down to the smallest detail.$\setminus$n
3. Explicit Constraints: Define the limitations or boundaries of the task through explicit examples, steps, or do's and don'ts.$\setminus$n
4. Mechanical Adherence: Stress the importance of formal aspects that need to be strictly followed, such as deadlines, word counts, or other formal criteria.$\setminus$n$\setminus$n

The goal of the Universiality-only instruction is to generate output that semantically acceptable  within the given context, without any restriction on the response. On the other hand, the goal of Conformity-only instruction is to generate strictly and precisely adhere to the given response guidelines, without considering the semantic meanings. Note that you should maintain the overall tone and style of the original instruction.$\setminus$n$\setminus$n

\#\#\#
Input: You are given a question on high school mathematics. You are also given 4 answer options (associated with "A", "B", "C", "D"), out of which only one is correct. You need to answer the question by selecting the correct option. You should only answer with the choice letter, not the whole answer.$\setminus$n$\setminus$n

Output:$\setminus$n
1. You are given a question on high school mathematics. Your task is to solve it.$\setminus$n
2. You are provided with four labeled answer options, "A," "B," "C," and "D." Respond with only one letter among the answer options.$\setminus$n
\#\#\# 
Input: Find the movie name from the given conversation. If the movie name is not found give output as "unknown"$\setminus$n$\setminus$n

Output:$\setminus$n
1. Find the movie name from the given conversation.$\setminus$n
2. Answer with the movie name or "unknown".$\setminus$n
\#\#\#
Input: In this task, you are given Twitter posts. Your task is to label the post's emotion (as expressed by the user) as sadness, joy, love, anger, fear, or surprise.$\setminus$n$\setminus$n

Output:$\setminus$n
1. In this task, you are given Twitter posts. Your task is to label the post's emotion.$\setminus$n
2. In this task, your task is to answer with emotions among sadness, joy, love, anger, fear, or surprise.$\setminus$n$\setminus$n

\#\#\#
Input: You are given a short text as a title. Your task is to generate a poem as output that is related to the given title and should feel like written by kids. The output should be a run-on sentence (two or more complete sentences connected without any punctuation). The poem should not be too long or too complex, because it should feel like it is written by younger person without high level of literature education.$\setminus$n$\setminus$n

Output:$\setminus$n
1. You are given a short text as a title. Your task is to generate a poem as output that is related to the given title and should feel like written by kids. It should feel like it is written by younger person without high level of literature education.$\setminus$n
2. You are given a short text as a title. Your task is to generate a run-on sentence (two or more complete sentences connected without any punctuation) output. It  should not be too long or too complex.$\setminus$n
\#\#\#
Input: Classify the relation of question with context to one of these categories: 1) award received, 2) based on, collection, 3) conflict, 4) constellation, 5) convicted of, 6) date of death, 7) director, 8) drafted by, 9) educated at, 10) medical condition, 11) military branch, 12) narrative location, 13) occupation, 14) original network, 15) parent company, 16) point in time, 17) production company, 18) residence, 19) series, 20) service entry, 21) sex or gender, 22) spouse, 23) standards body question.$\setminus$n$\setminus$n

Output:$\setminus$n
1. Classify the relation of question with context.$\setminus$n
2. Answer with one of these categories: 1) award received, 2) based on, collection, 3) conflict, 4) constellation, 5) convicted of, 6) date of death, 7) director, 8) drafted by, 9) educated at, 10) medical condition, 11) military branch, 12) narrative location, 13) occupation, 14) original network, 15) parent company, 16) point in time, 17) production company, 18) residence, 19) series, 20) service entry, 21) sex or gender, 22) spouse, 23) standards body question.$\setminus$n
\#\#\#
Input: You are shown a random response (from a computer or a human). Generate a language query such that it leads to this reply.$\setminus$n$\setminus$n

Output:$\setminus$n
1. You are shown a random response (from a computer or a human). Generate a query that corresponds to the given reply.$\setminus$n
2. The response you are shown may come from either a computer or a human. Generate a precise language query in a manner that would elicit the given reply specifically.$\setminus$n
\#\#\#
Input: {definition}$\setminus$n
Output:$\setminus$n
1.
\end{tabular}
\label{tab:prompt_for_generate_instructions}
\end{table}


==> old/02-problem-statement.tex <==
\section{Problem Statement}
\label{sec2:problem_statement}

\paragraph{Notations}
% the goal of language model 
We \( x_{i:j} \) represent a sequence that starts with the $i$-th element \( x(i) \) and ends with \( x(j) \). The shorthand \( x_j \) is equivalent to \( x_{1:j} \), where the starting index is omitted for brevity. To distinguish between multiple sequences, we use superscripts, such as \( x^1_t \) and \( x^2_t \), both of which are sequences of length \( t \). The set \([n]\) consists of integers from 1 to \( n \).

Consider the auto-regressive LM $\mathcal{M}_{\theta}$, parameterized by $\theta$. In the zero-shot scenario, the model takes an instruction $I_{<s}$ and a context $x_{x<t}$, and then generates subsequent tokens $x_{t+1}$, $x_{t+2}, \cdots$ as:

\begin{equation}
    %x(t+1) \sim 
    p_{\theta}(x_{t+1}) = \mathcal{M}_{\theta}(x_{t+1}| I_{<s}, x_{<t}) \quad \text{where } x \in \Omega.
\end{equation}

Here, $\Omega$ represents the set of all possible vocabulary tokens. The next token is determined by the distribution $\mathcal{M}(\cdot | x_t)$. It can either be the token with the highest probability (i.e., greedy decoding) or sampled from its temperature-scaled distribution (i.e., sampling).

In the few-shot setting, demonstration examples are combined into $I$. Note that the natural language instruction $I$ can vary in both its inherent semantics and superficial formats. From now on, we use $p_{\theta}(x)$ and $q_{\tilde{\theta}}(x)$ to specify the distributions from $\mathcal{M}_{\theta}$ and $\mathcal{M}_{\tilde{\theta}}$, each adjusted according to the specific decoding method used.

%\paragraph{Evaluation of Instruction-Based Responses} 


% Understanding the ability of instruction following is a challenging task. In the wider context, this capability is alluded to in an offhand manner, paving the way for varied interpretations, a phenomenon we refer to as the \textit{anchoring effect} where the models rely heavily on the \textbf{first piece of information} (the ``anchor") in the generation phase\,\citep{coherence_boosting}. 


% \begin{itemize}
%     \item \textbf{Precise Match (PM):} This measures the accuracy (e.g., exact match) or similarity (e.g., ROUGE-L) between the output and the golden label (perfect adherence to the instruction).

%     \item \textbf{Instruction Conformity (IC):} While the output might not match the golden label verbatim, it remains within the instruction-guided output space (e.g., `True' and `False'). An example would be when the golden label dictates `True', but the output responds with `False'.

%     \item \textbf{Semantic Coherence (SC):} This metric captures instances where the output, though not an exact match to the golden label, still retains semantic congruence with the intended instruction. For instance, responding with `true' in lowercase or offering a synonym like `correct' in lieu of the precise term.
% \end{itemize}

% The symbol \( x(i) \) refers to the $i$-th element of sequence \( x \). To differentiate among various sequences, we use subscripts. As an example, \( x^1_t \) and \( x^2_t \) stand for two separate sequences, both of length \( t \). The notation \([n]\) represents the set of integers from 1 up to \( n \).

% Consider a generative LM parameterized by $\theta$. In general zero-shot setting, during inference with given an instruction $I_s$ and a context $x_t$, an autoregressive language model $\mathcal{M}_{\theta}$ parameterized by $\theta$ generates successive tokens $x(t+1), x(t+2), ...$:

% \begin{equation}
%     x(t+1) \sim p_{\theta}(x) = \mathcal{M}_{\theta}(x | I_s, x_t) \quad \text{where } x \in \Omega
% \end{equation}

% where $\Omega$ is the vocabulary. The output token is drawn from the temperature-scaled distribution $\mathcal{M}(\cdot | x_t)$ (e.g., the next token is selected following the maximum likelihood method when the temperature is zero; \textit{greedy-decoding}).
% % either choosing the argmax probability (i.e. greedy manner) or sampled from probability distribution (i.e. sampling manner). 
% In few-shot setting, the demonstration examples are concatenated into $I$. Note that the natural language instruction $I$ may have diverse forms in both its inherent semantics and superficial formats. Going forward we will assume that $p_{\theta}(x)$ and $q_{\tilde{\theta}}(x)$ denotes the distributions from $\mathcal{M}_{\theta}$ and $\mathcal{M}_{\tilde{\theta}}$ respectively, adjusted for the sampling method.

% % \input{materials/tables/table_benchmark}

% % \paragraph{Capacity of Instruction Following.} 
% Understanding the ability of instruction following is a challenging task. In the wider context, this capability is alluded to in an offhand manner, paving the way for varied interpretations, a phenomenon we refer to as the \textit{anchoring effect} where the models rely heavily on the \textbf{first piece of information} (the ``anchor") in the generation phase\,\citep{coherence_boosting}. In this work, we explore the ways in which a language model generates its responses anchored by the given instruction. To evaluate the extent of alignment between models' responses and prescribed instructions, we introduce the subsequent evaluative metrics:

% \begin{itemize}
%     \item \textbf{Precise Match (PM):} This measures the accuracy (e.g., exact match) or similarity (e.g., ROUGE-L) between the output and the golden label (perfect adherence to the instruction).

%     \item \textbf{Instruction Conformity (IC):} While the output might not match the golden label verbatim, it remains within the instruction-guided output space (e.g., `True' and `False'). An example would be when the golden label dictates `True', but the output responds with `False'.

%     \item \textbf{Semantic Coherence (SC):} This metric captures instances where the output, though not an exact match to the golden label, still retains semantic congruence with the intended instruction. For instance, responding with `true' in lowercase or offering a synonym like `correct' in lieu of the precise term.
% \end{itemize}

%=======================================================
% When conditioned upon a given anchor (instruction), the model engages in a delicate balancing act, oscillating between two primary modes of operation: universality and conformity. Each of these modes defines distinct characteristics to the model's responses:

% \paragraph{Illustrative Examples.} To further clarify universality and conformity, we provide concrete examples that demonstrate each mode of response within a language model context (\autoref{tab:usecase}):

% \input{materials/tables/table_usecases}

% \begin{itemize}
%     \item \textbf{AC task}: Models are presented with a Wikipedia excerpt and a related query. Without explicit instruction, a model might lean on universality, gravitating towards notable entities in the text for answers, as evidenced by the uninstructed output of `FBI'. However, with a clear directive to determine answerability, the model’s response is more in line with conformity, judiciously evaluating the context against the query to produce a more binary `True' or `False' output.
%     \item \textbf{WA task}: The WA task demands a different kind of reasoning. Absent a specific directive, the model taps into its universality. Given `stir : spoon', it draws upon broad associations; stirring often invokes the imagery of a spoon. Hence, when tasked with `cut', it naturally offers ``knife'', a prevalent association. However, when guided by a detailed instruction, there's a distinct shift. Instead of just relying on generalized knowledge, the model embraces conformity, considering an array of tools associated with `cut', exploring beyond the immediate and encompassing options like `scissors', `sword', and `glass'.
% \end{itemize}

% These tasks, while diverse, underscore a shared narrative: The adaptability of PLMs in oscillating between the broad-ranging grasp of universality and the precision of conformity.


% \begin{figure}[t]
% \begin{center}
%    \includegraphics[width=1.0\linewidth]{materials/figures/EM_SC_IC_3b_11b.pdf}
% \end{center}
% \caption{Performance comparison of Tk-\textsc{Instruct} models over 58 unseen classification tasks in the \textsc{SupNatInst} dataset.}
% \label{fig:em_sc_ic_3b_11b}
% \end{figure}

% \begin{table}[t]
% \centering
% \caption{Performance comparison of Tk-\textsc{Instruct} models over 58 unseen classification tasks in the \textsc{SupNatInst} dataset. The table shows EM and SC scores as a fraction of IC. Further columns represent the count of tasks where IC is precisely 0.0, exceeds 0.90, and surpasses 0.99, respectively.}
% \label{tab:pilot_tk_instruct}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lccccc@{}}
% \toprule
% Models          & Avg. EM / IC & Avg. SC / IC & $\sum_{task\,\mathcal{T}} \mathbb{1}[\text{IC}_{task\,\mathcal{T}} = 0.]$ & $\sum_{task\,\mathcal{T}} \mathbb{1}[\text{IC}_{task\,\mathcal{T}} > 90.00]$ & $\sum_{task\,\mathcal{T}} \mathbb{1}[\text{IC}_{task\,\mathcal{T}} > 99.00]$ \\ \midrule
% Tk-\textsc{Instruct}-3b  & 54.30   & 84.80   & 6            & 41                  & 34                   \\
% Tk-\textsc{Instruct}-11b & 58.90   & 84.82   & 4            & 35                  & 25                   \\ \bottomrule
% \end{tabular}
% }
% \end{table}










% \paragraph{Validation for Pretrained Tk-\textsc{Instruct} Models with the Variants of Instructions.} 
% key motivation for the Instructive Decoding
% Noisy Instruction에 대한 Top5 Probablity token을 살펴보고, 이것을 어떻게 정제할 수 있는지를 살펴본다. 

% \autoref{fig:em_sc_ic_3b_11b} present the performance of two prominent Tk-\textsc{Instruct} models across 58 unseen classification tasks from the \textsc{SupNatInst} dataset, assessed using our metrics. As evidence, while conventional metrics might hint at model inaccuracies, our introduced metrics - IC and SC\,\footnote{\autoref{fig:em_sc_ic_3b_11b} and \autoref{tab:pilot_tk_instruct} are evaluated by creating a semantic coherent label set for each task. Detailed information is in the appendix.} - highlight the models' capacities to provide semantically coherent and instruction-conformant responses, even when they do not achieve a direct match. Through these multiple evaluations, we can observe the following patterns:


==> old/_backup_tex <==

% Language Models\,(LMs) have significantly advanced the field of Natural Language Processing\,(NLP)\,\citep{llm_survey, gpt4_report}, as a result of extensive pre-training on vast datasets and the use of billions of parameters\,\citep{scaling_law}. These models exhibit emergent abilities\,\citep{emergent_abilities_llms}, especially in tasks demanding complex reasoning or understanding. One such distinguished is In-Context Learning\,(ICL), where LMs generate responses by leveraging a few demonstration examples within their input prompts, eliminating the need for additional parameter updates\,\citep{gpt3, icl_survey}. Further exploration in this direction leads us to instruction-following models, adept at aligning their responses seamlessly with human-like expectations, setting the stage for more collaborative AI-human interactions\,\citep{instruction_tuning_survey, align_survey, interactive_survey}.

% Instruction-tuning\,\citep{flan, t0} presents a straightforward approach to enhance the instruction following of LMs. While LMs, through extensive pre-training, amass a vast knowledge reservoir, they may not always generate outputs aligned with specific user intents. By fine-tuning these models on diverse tasks framed as natural language instructions, instruction-tuning directs the model's underlying knowledge to generate outputs more precisely aligned with users' expectations\,\citep{gpt3, lms_are_unsupervised_multitask_learners}. As evidence, instruction-tuned models exhibit superior performance in generating contextually relevant responses in zero-shot scenarios\,\citep{sni_dataset, instruction_tuning_with_gpt4}. Recent studies underscore the critical role of instruction-tuning in enabling LMs to effectively guide their pre-trained knowledge to diverse problems\,\citep{instruct_gpt, flan_t5}.
%------
% By fine-tuning an LM on a wide range of tasks phrased as the formatted instructions, instruction-tuning effectively relieves the mismatch between pre-training objectives\,(e.g., next token prediction) and human user's objectives\,\citep{gopher, gpt3, lms_are_unsupervised_multitask_learners}. 

% As a consequence, the instruction-tuned models can generate desired responses in the zero-shot scenarios\,\citep{sni_dataset, instruction_tuning_with_gpt4}. 


% However, instruction-tuned models occasionally falter in consistently adhering to instructions, particularly for unfamiliar tasks. This divergence from the expected output can be attributed to the inherent limitations of the training datasets, be they human-annotated\,\citep{ni_dataset, sni_dataset} or model-generated\,\citep{self_instruct, unnatural_ni_dataset}. Refining these datasets, while pivotal, often comes with considerable manual effort or computational overhead, underscoring the need for a more streamlined approach\,\citep{flan_t5, lima}. Furthermore, the intricacies of how these models interpret and respond to instructions remain an active area of inquiry. Recent research has begun to shed light on this\,\citep{did_you_read_instructions, instruction_verbalizer_manipulation, evaluating_robustness_instruction_tuned}, yet a comprehensive understanding of the models' interactions with diverse instructions is still a frontier\,\citep{llm_counterfactual_tasks, do_really_understand_prompts, instructeval}. Although `prompt-engineering' techniques like rephrasing\,\citep{prompt_phrase} or stochastic sampling methods (e.g., temperature sampling)\,\citep{self_consistency} have been introduced to diversify responses and address these challenges, their efficacy often relies on fortuitously finding the apt prompt for a given task or extracting well-suited responses across multiple seeds, making them somewhat fortuitous in nature.

% However, instruction-tuned models frequently struggle to follow instructions when they encounter \textit{unseen} tasks, often generating responses that deviate from the intended task objectives. 
% Although previous studies have improved instruction-tuning by using diverse task datasets that are either human-annotated\,\citep{ni_dataset, sni_dataset} or model-generated\,\citep{self_instruct, unnatural_ni_dataset}, these methods are either labor-intensive or computationally demanding. They often require manual oversight to ensure both the quality and diversity of the instructions used for tuning\,\citep{flan_t5, lima}. 
% Moreover, there remains a lack of understanding regarding how instructions influence the responses of instruction-tuned models\,\citep{did_you_read_instructions, instruction_verbalizer_manipulation, evaluating_robustness_instruction_tuned}, as well as how these models interpret and act upon the given instructions\,\citep{llm_counterfactual_tasks, do_really_understand_prompts, instructeval}.

% In light of these difficulties, the concept of contrastive decoding emerges as a potential solution\,\citep{contrastive_decoding, contrastive_input_decoding}. The underlying principle is to leverage the disparity between predictions of primary models and alternative `amateur' models, generating fluent and lexically diverse text.



% the anchoring effect\,\citep{kahneman1982judgment}—a cognitive bias wherein models heavily rely on the first piece of information encountered—has investigated as an intriguing solution to adjust the outputs generated by LMs\,\citep{jones2022capturing}. The potential of harnessing this effect in the context of LMs, particularly within the contrastive decoding paradigm, is a compelling proposition\,\citep{contrastive_decoding, contrastive_input_decoding}. By emphasizing the initial instructions and contrasting them with alternative `amateur' models, we can guide models towards generating more fluent and lexically diverse text while staying true to the task's essence.
% (i.e., a phenomenon where the models rely heavily on the \textbf{first piece of information} in the generation phase\,\citep{kahneman1982judgment, coherence_boosting, jones2022capturing})



%: randomly shortening\,(\textit{random truncate}), replacing it with a misleading prompt\,(\textit{opposite}), randomly generated words\,(\textit{random words}) or omitting it entirely\,(\textit{null}). % "These noisy instructions distract the model, leading it to predict next-token logits that deviate from the original instruction. We demonstrate that ID leverages this discrepancy to adjust the decoding process, contrasting the original next-token logits with those generated under the influence of the noisy instructions."


% that refines the focus of instruction-tuned LMs on the given instruction during generation. 
% ID distracts or distorts the original instruction by replacing it with the following \textit{noisy} variants: randomly shortening\,(\textit{random truncate}), replacing it with a misleading prompt\,(\textit{opposite}), randomly generated words\,(\textit{random words}) or omitting it entirely\,(\textit{null}). These noisy instructions distract the model, leading it to predict next-token logits that deviate from the original instruction. We demonstrate that ID leverages this discrepancy to adjust the decoding process, contrasting the original next-token logits with those generated under the influence of the noisy instructions.


% This ability has been further explored to follow the natural language instructions\,\citep{instruct_gpt, instruction_tuning_survey}, thereby the generated responses to be better aligned with human expectations\,\citep{align_survey, interactive_survey}.


%To address these gaps, we introduce an innovative approach: \textit{instructive decoding}\,(\autoref{fig:main}). This method leverages the inconsistencies introduced by given instructions to sharpen the responses of instruction-tuned models. Conceptualized in a contrastive manner, instructive decoding samples the output logit for the upcoming word from a probability distribution derived from the logit disparities between base responses and those influenced by certain perturbed instructions (i.e., truncating specific words from the original instruction). By cross-referencing flawed responses steered by these modified instructions, we can mitigate semantic noise (e.g., where the correct label is `True', but the model outputs `Correct' or `Positive'). This method not only boosts \textit{instruction conformity} but also nudges models towards more accurate and factual responses.

% We propose to exploit the overriding from the given instruction to refine the responses of instruction-tuned models in a contrastive manner, termed as \textit{instructive decoding}, where the output logit over the next word is sampled from the probability of logit differences obtained from base responses versus the responses guided by certain noisy instructions (i.e., certain words in the given instruction is truncated). By removing the semantic noise (e.g., instruction label should be `True', but the model response is `Correct' or `Positive') by referring to the wrong answers guided by noisy instruction, we can potentially enhance the models not only having higher \textit{instruction conformity} but also making more factual response.

%Many studies demonstrate that advancing instruction tuning by scaling model size and task numbers, and incorporating chain-of-thought datasets significantly enhances performance across various benchmarks and evaluations, setting new state-of-the-art results\,\citep{flan_t5}.
%Despite its simplicity of scaling, the computational demands are substantial, and the need for manual oversight to ensure the quality and diversity of outputs is undeniable. 
%To harness the full potential of these models, it should be understood how instruction-tuned models identify the instruction and align their response to the given instructions\,\citep{instructeval, how_far_can_camels_go}.
%Instruction-tuned models struggle when the given instructions or anticipated outcomes override their pretrained semantic knowledge\,\citep{instruction_verbalizer_manipulation, llm_counterfactual_tasks, do_really_understand_prompts}. 
%For example, enforcing the models to respond `negative' to the positive statement significantly degrades the performance\,\citep{instruction_verbalizer_manipulation}. The models also encounter difficulties when responding to instructions that have different formats from those they observed during the instruction-tuning phase\,\citep{evaluating_robustness_instruction_tuned, formatting_consistency}. 
%While previous studies have made strides, thanks to diverse task datasets assembled through human-annotation\,\citep{ni_dataset, sni_dataset} and model-driven techniques\,\citep{self_instruct, unnatural_ni_dataset}, there is still much to recognize the behavior of instruction-tuned models\,\citep{did_you_read_instructions, controllable_generation_survey}. 

% To address these gaps, we introduce an innovative approach: \textit{instructive decoding}\,(\autoref{fig:main}). This method leverages the inconsistencies introduced by given instructions to sharpen the responses of instruction-tuned models. Conceptualized in a contrastive manner, instructive decoding samples the output logit for the upcoming word from a probability distribution derived from the logit disparities between base responses and those influenced by certain perturbed instructions (i.e., truncating specific words from the original instruction). By cross-referencing flawed responses steered by these modified instructions, we can mitigate semantic noise (e.g., where the correct label is `True', but the model outputs `Correct' or `Positive'). This method not only boosts \textit{instruction conformity} but also nudges models towards more accurate and factual responses.

% We propose to exploit the overriding from the given instruction to refine the responses of instruction-tuned models in a contrastive manner, termed as \textit{instructive decoding}, where the output logit over the next word is sampled from the probability of logit differences obtained from base responses versus the responses guided by certain noisy instructions (i.e., certain words in the given instruction is truncated). By removing the semantic noise (e.g., instruction label should be `True', but the model response is `Correct' or `Positive') by referring to the wrong answers guided by noisy instruction, we can potentially enhance the models not only having higher \textit{instruction conformity} but also making more factual response.


%Examples of outputs that achieve either Universality or Conformity. Highlighted elements in the instruction identify the contributing factors for each component. \textbf{Output (a)} achieves Universality as it implies the question is answerable, but lacks Conformity due to its incorrect format. \textbf{Output (b)} achieves Conformity as it meets the format requirements, but lacks Universality due to its incorrect content. \textbf{Output (c)} satisfies both Universality and Conformity.

% In this paper, we present two key dimensions to understand the alignment of generated outputs with given instructions: \textbf{Universality} and \textbf{Conformity} (\S\,\ref{sec2}). For universality, the outputs should be semantically aligned to the context given by the instruction, utilizing the model's pre-trained knowledge (i.e., semantic coherence between input and its response). For conformity, the output should strictly adhere to the rules or guidelines described in the instruction, adapting the output to meet the specific needs of the task. \autoref{fig:uni_conf_output_example} provides examples of outputs that achieve either Universality or Conformity for the given instruction.
%==================== MEthod ===================================

% The essence of ID revolves around the manipulation of a model's response, leading to pronounced contrasts during the decoding process. Such a strategy guarantees a closer alignment with instructions, promising enhanced generalization across diverse tasks and challenging established norms. 
% To delve deeper into the mechanics, this method contrasts logits, particularly differentiating between \(z_p\)—originating from the base instruction, and \(z_q\)—emerging from its noisy version. This contrast fine-tunes token predictions, ensuring that the model's generated output mirrors the intended instruction as described in Algorithm~\ref{algorithm}.


% instruction을 의도적으로 noisy하게 만들어서 instruction과 관련 없는 뒤의 input과 model에 bias된 output을 유도해서, 이를 기존 prediction에서 contrastive 하게 활용하면 충분히 좋은 접근이 될수 있다.


% proposes a novel avenue to enhance LMs' alignment with given instructions. Given the nuanced hurdles posed by unseen task generalization and noting that smaller amateur models don't uniformly underachieve compared to their larger peers, the course of action is evident: harnessing this cognitive trait may pave the way for a groundbreaking refinement in instruction-tuned LMs.

% To alleviate these challenges, we introduce \textit{Instructive Decoding} (ID), a simple yet effective method to amplify the focus of instruction-tuned LMs on provided instructions during the generation phase. Central to ID is the inception of \textit{noisy} variants, specifically curated to instigate an \textit{anchoring effect} — a cognitive bias in behavioral phenomenon wherein models tend to anchor the \textbf{first piece of information} presented\,\citep{kahneman1982judgment, coherence_boosting, jones2022capturing}. Importantly, we diverge from the convention of relying on smaller amateur models, which do not universally underperform compared to larger models across all task categories for unseen task generalization. Instead, we underline the potency of prompt engineering. By manipulating a model's response to yield more divergent outcomes, we can introduce a pronounced contrast during the decoding process. This approach not only ensures a tighter alignment with the provided instructions but also promises enhanced generalization across a variety of tasks, challenging the established norms in model reliance and decoding methodologies. Specifically, this process involves contrasting logits distinguishing between \(z_p\), derived from the foundational instruction, and \(z_q\), formed from its noisier counterpart. The resulting contrast finely tunes token predictions, ensuring the model's output remains faithful to the intended instruction (Algorithm~\ref{algorithm}).


% Building upon the concept of the \textit{anchoring effect} from behavioral economics, our method, ID, emphasizes the importance of grounding model predictions. We present a novel strategy: juxtapose the provided instruction with a slightly modified or distorted variant, which triggers contrastive decoding within the model. This technique is designed to hone the model's comprehension of the initial instruction. By intermittently omitting certain elements or introducing off-track anchors, we mold LMs to generate more plausible and contextually apt responses. This process involves contrasting logits, specifically, distinguishing between \(z_p\), derived from the foundational instruction, and \(z_q\), formed from its noisier counterpart. The resulting contrast finely tunes token predictions, ensuring the model's output remains faithful to the intended instruction (Algorithm~\ref{algorithm}).

% \paragraph{Implementation.} As illustrated in Algorithm~\ref{algorithm}, our ID method refines model outputs for better alignment with given instructions. It begins by acquiring logits, $z^p$ and $z^q$, for each token position $n$ until the target sequence length $T$, using both a base instruction and a noisy counterpart. The model then constructs the next token's prediction by contrasting these logits, thereby subtly rectifying potential prediction inaccuracies and ensuring a closer adherence to the base instruction.


